Piet: Facilitating Color Authoring for Motion Graphics Video

Motion graphic (MG) videos are effective and compelling for presenting complex concepts through animated visuals; and colors are important to convey desired emotions, maintain visual continuity, and signal narrative transitions. However, current video color authoring workflows are fragmented, lacking contextual previews, hindering rapid theme adjustments, and not aligning with progressive authoring flows of designers. To bridge this gap, we introduce Piet, the first tool tailored for MG video color authoring. Piet features an interactive palette to visually represent color distributions, support controllable focus levels, and enable quick theme probing via grouped color shifts. We interviewed 6 domain experts to identify the frustrations in current tools and inform the design of Piet. An in-lab user study with 13 expert designers showed that Piet effectively simplified the MG video color authoring and reduced the friction in creative color theme exploration.

==> texfiles/4-design_goals.tex <==
\section{Design Goals and Rationale}
Driven by the observed challenges in MG video color authoring and our discussions with motion graphics professionals, we derive the following design goals to address the challenges in MG video color authoring and guide the development of \sysname{}. 
\begin{itemize}[leftmargin=2em]
    \item[\textbf{D1.}] \textbf{Integrate color editing with video playback for real-time contextual feedback.}
    The temporal nature of MG videos requires a continuous and cohesive narrative. 
    By merging color editing with video playback, designers can immediately see how color changes impact the storyline. 
    This not only speeds up the design process but also ensures that the narrative flow remains undisturbed by color modifications.
    \item[\textbf{D2.}] \textbf{Enable both individual and group-wise color adjustments.}
    In MG video authoring, designers have dual needs: refining individual elements and harmonizing colors across multiple elements for style consistency. 
    This balance stems from two distinct design perspectives: the \emph{object-driven} focus on isolated components, and the \emph{scene-driven} approach, which emphasizes holistic visual cohesion. 
    To support both, it's crucial to offer different views that highlight individual objects and the overall color palette within scenes. 
    By facilitating both types of adjustments, we simplify the editing process, enabling designers to swiftly transition between detailed tweaks and broad thematic edits.
    \item[\textbf{D3.}] \textbf{Present an overview of color distribution with adjustable detail levels.}
    Understanding the color distribution in a video is important for informed color design decisions and prioritizing designers' edits. 
    Our study indicates that color dominance in an MG video hinges on its visual presence and recurrence across frames. 
    Therefore, it's essential to ensure these aspects are reflected in the color distribution overview. 
    In addition, an adjustable overview is necessary to allow designers to zoom in on specifics or zoom out for a broader perspective, giving them flexibility in how they approach and execute their color adjustments.
\end{itemize}
